Chain-of-Thought Embeddings for Stance Detection on Social Media

Stance detection on social media is challenging for Large Language Models (LLMs), as emerging slang and colloquial language in online conversations often contain deeply implicit stance labels. Chain-of-Thought (COT) prompting has recently been shown to improve performance on stance detection tasks -- alleviating some of these issues. However, COT prompting still struggles with implicit stance identification. This challenge arises because many samples are initially challenging to comprehend before a model becomes familiar with the slang and evolving knowledge related to different topics, all of which need to be acquired through the training data. In this study, we address this problem by introducing COT Embeddings which improve COT performance on stance detection tasks by embedding COT reasonings and integrating them into a traditional RoBERTa-based stance detection pipeline. Our analysis demonstrates that 1) text encoders can leverage COT reasonings with minor errors or hallucinations that would otherwise distort the COT output label. 2) Text encoders can overlook misleading COT reasoning when a sample's prediction heavily depends on domain-specific patterns. Our model achieves SOTA performance on multiple stance detection datasets collected from social media.

==> Sections/ErrorAnalysis.tex <==
\section{Where Does ChatGPT Fail on STS?} \label{err_analysis}
In this section, we analyze the top 500 most poorly predicted samples from ChatGPT (i.e. largest absolute difference between prediction and ground truth) across the STS12-16 and STS-B in the 0-shot setting. Our goal is to quantitatively support various claims regarding the types of text pairs not well suited for semantic similarity modeling with ChatGPT. We specifically discuss ChatGPT's struggle with linguistically unacceptable texts and numeric comparisons.  

\subsection{Linguistic Acceptability}

We qualitatively observed that ChatGPT struggles with samples which are syntactically or grammatically incoherent. We validate this claim by running a RoBERTa-base model fine-tuned on the COLA \cite{warstadt2018neural} dataset, which tests if a text is linguistically acceptable. We find that \textbf{33.4\% of highly inaccurate predictions contain a linguistically unacceptable text}. For example, consider the following sample from STS14:\\ \noindent \textbf{Text 1:} what isn 't how what was sold ? \\\textbf{Text 2: }it 's not how it was sold , gb. \\\textbf{Ground Truth Similarity Score:} 0.32\\ 
ChatGPT has very little content or semantics to rely on when analyzing two linguistically unacceptable texts. Thus, it cites the presence of common words such as ``isn't," ``how," and ``sold" when assigning an incorrectly high similarity score of 0.75. 

\subsection{Numeric Reasoning}
It is well-documented that large language models have trouble with numeric reasoning tasks \cite{chen2023need}. We find that ChatGPT is not very sensitive to differences in numeric quantities when analyzing the semantic equivalence of texts. In other words, ChatGPT commonly gives high semantic equivalence to linguistically similar texts with very different numeric quantities. We specifically find that, of the top-500 worst predictions made by ChatGPT, \textbf{14.6\% require a numeric comparison}. Consider the following example: \\
\noindent \textbf{Text 1:} 	singapore stocks end up 0.26 percent \\\textbf{Text 2:} singapore stocks end up 0.11 pct \\\textbf{Ground Truth 
 Similarity Score:} 0.4\\ 
ChatGPT is good at recognizing that both texts pertain to a Singapore stocks, however ChatGPT's prediction of 0.95 similarity shows little sensitivity to the numeric difference between the texts. 
